Quantitative inverse problem in visco-acoustic media under attenuation model uncertainty

We consider the inverse problem of quantitative reconstruction of properties (e.g., bulk modulus, density) of visco-acoustic materials based on measurements of responding waves after stimulation of the medium. Numerical reconstruction is performed by an iterative minimization algorithm. Firstly, we investigate the robustness of the algorithm with respect to attenuation model uncertainty, that is, when different attenuation models are used to simulate synthetic observation data and for the inversion, respectively. Secondly, to handle data-sets with multiple reflections generated by wall boundaries around the domain, we perform inversion using complex frequencies, and show that it offers a robust framework that alleviates the difficulties of multiple reflections. To illustrate the efficiency of the algorithm, we perform numerical simulations of ultrasound imaging experiments to reconstruct a synthetic breast sample that contains an inclusion of high-contrast properties. We perform experiments in two and three dimensions, where the latter also serves to demonstrate the numerical feasibility in a large-scale configuration.

==> sections/5-numerical-inversion.tex <==
%% -----------------------------------------------------------
\section{Experiments of medical imaging in viscoacoustic media}
% for the pictures only in the area of interest
\pgfmathsetmacro{\xminloc} {2.80}
\pgfmathsetmacro{\xmaxloc}{15.50}
\pgfmathsetmacro{\zminloc} {2.80}
\pgfmathsetmacro{\zmaxloc}{15.50}
%% -----------------------------------------------------------


We carry out the reconstruction algorithm and only 
investigate the recovery of the wave-speed $c_0$.
While the density and attenuation coefficient are \emph{not} 
known initially, we do not recover them as the data are less 
sensitive to their variations (e.g., \cite{Faucher2017}). 
The initial models for the reconstruction correspond
to homogeneous background with 
\begin{equation}
  c_0   \,= \, \num{1490} \si{\meter\per\second} \, , \qquad
  \rho \, = \, \num{1000} \si{\kg\per\meter\cubed}, \qquad
  \text{constant initial models for inversion.}
\end{equation} 

We consider multi-frequency data and use $5$ frequencies for 
the reconstruction: from $500$ \si{\kilo\Hz} to $1$ \si{\mega\Hz}, 
every $100$ \si{\kilo\Hz}. 
For each individual frequency, \num{40} minimization iterations 
are carried out and the reconstruction obtained at the current
frequency is used as initial guess for the next one. 

%% ---------------------------------
\setlength{\modelwidth} {6.50cm}
\setlength{\modelheight}{6.50cm}
\graphicspath{{figures/tumor_18x18/main/}}
%% ---------------------------------
\begin{figure}[ht!] \centering
\renewcommand{\modelfile}{cp-homogeneous_1470-1550}
%\subfloat[][Initial constant wave-speed model, set to \num{1490} \si{\meter\per\second}.]
%           {\input{figures/tumor_18x18/skeleton-full_cp}
%            \label{fig:initial-guess:cst-cp}}
%\renewcommand{\modelfile}{rho-homogeneous_0.8-1.12}
%\subfloat[][Initial constant density model, set to \num{1000} \si{\kg\per\meter\cubed}.]
%           {\input{figures/tumor_18x18/skeleton-full_rho}
%            \label{fig:initial-guess:cst-rho}}
\caption{The initial guesses for the reconstruction: we consider homogeneous, 
         constant wave speed and density.}
\label{fig:initial-guess}
\end{figure}

% ---------------------------------------------------
\subsection{Synthetic data with two levels of noise}
% --------------------------------------------------

To carry out the inverse scheme, we generate synthetic data 
depending on the acquisition setups described in \cref{section:acquisition-setup}.
Despite having synthetic data, we incorporate noise to 
produce a more realistic configurations. Namely, we 
include noise at two levels: 
\begin{enumerate}
  \item We use noisy models to generate the data, these are illustrated in \cref{fig:noise-models}.
  \item Once the data are generated with from the noisy model, we incorporate noise in the 
        resulting signals.
\end{enumerate}
\todoflo[inline]{Illustrate the data-set.}

%% ---------------------------------
\setlength{\modelwidth} {6.50cm}
\setlength{\modelheight}{6.50cm}
\graphicspath{{figures/tumor_18x18/main/}}
%% ---------------------------------
\begin{figure}[ht!] \centering
%\renewcommand{\modelfile}{cp-tumor-noise-v2_1470-1550}
%\subfloat[][The wave speed model with noise used to generate the synthetic data.]
%           {\input{figures/tumor_18x18/skeleton-full_cp}}
%\renewcommand{\modelfile}{rho-tumor-noise-v2_0.8-1.12}
%\subfloat[][The density model with noise used to generate the synthetic data.]
%           {\input{figures/tumor_18x18/skeleton-full_rho}}
\caption{The wave speed and density models with included noise that are used to generate the synthetic data.}
\label{fig:noise-models}
\end{figure}
%% ---------------------------------


% ========================================
\subsection{Reconstructions}
% ========================================

In the following, we show the reconstructions of the wave-speed 
depending on the acquisition setup, the positions of the receivers
and the attenuation models. We have: 
\begin{itemize}
  \item nine configurations for the acquisition setup, cf.~\cref{subsection:summary-benchmark}.
  \item five possibilities for the attenuation model used to generate the data: 
        \cref{eq:kolsky-futterman,eq:zener,eq:kelvin-voigt,eq:maxwell,eq:cole}.
  \item five possibilities for the attenuation model used during the inversion scheme: 
        \cref{eq:kolsky-futterman,eq:zener,eq:kelvin-voigt,eq:maxwell,eq:cole}.
\end{itemize}
Therefore, we have a total of \num{225} experiments, and most of them 
include `model error': when the model of attenuation used to generate
the data is different from the one used to carry out the reconstruction.


We illustrate the reconstructions depending on the choice the acquisition
setup in \cref{fig:fwi:all}. Here, the data are generated using the Zener
model \cref{eq:zener} while the reconstruction is performed with the 
Kelvin--Voigt attenuation model \cref{eq:kelvin-voigt}.

%% ---------------------------------
\setlength{\modelwidth} {5.00cm}
\setlength{\modelheight}{5.00cm}
\graphicspath{{figures/tumor_18x18/fwi/}} 
% 1: maxwell
% 2: cole-cole
% 3: kolsky-futterman
% 4: kelving-voigt
% 5: zener
%% ---------------------------------
\begin{figure}[ht!] \centering
\renewcommand{\bench}{SpwRskin}     \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSpwRs.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SpwRdisk}     \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSpwRd.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SskinRskin}   \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSskRs.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}}
%%%===========================
%\renewcommand{\bench}{SskinRbox}    \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSskRb.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SdiskRdisk}   \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSdkRd.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SdiskRbox}    \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSdkRb.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}}
%%%===========================
%\renewcommand{\bench}{SarrayRskin}  \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSarRs.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SarrayRbox}   \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSarRb.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}} \hfill
%\renewcommand{\bench}{SarrayRmove}  \renewcommand{\modelfile}{\bench_data-ZE_1MHz_Gauss2-4}
%\subfloat[][\benchSarRa.]
%           {\input{figures/tumor_18x18/skeleton-reduc_cp}}
\caption{Reconstruction using $5$ frequencies from 
         $500$ \si{\kilo\Hz} to 1 \si{\mega\Hz} 
         depending on the acquisition setup and starting
         from the constant background models displayed 
         in \cref{fig:initial-guess}. 
         The synthetic data are computed using the noisy
         models of \cref{fig:noise-models} and the Zener
         attenuation model. However, the reconstruction
         uses the Kelvin--Voigt attenuation model.
         We restrict the pictures to the area of interest 
         near the sample, between $x=\xminloc~\si{\centi\meter}$
         and $x=\xmaxloc~\si{\centi\meter}$ and 
         between $z=\zminloc~\si{\centi\meter}$
         and $z=\zmaxloc~\si{\centi\meter}$.}
\label{fig:fwi:all}
\end{figure}


To evaluate the performance of the reconstructions, 
we define the relative error norm of the models, defined by 
\begin{equation} \label{eq:relative-error}
  \mathfrak{e}(c_\mathrm{rec}) \,=\, 
  \Big\Vert \,\,  \dfrac{c_\mathrm{true} \,-\, c_\mathrm{rec}}{c_\mathrm{true}} \,\, \Big\Vert \, ,
\end{equation}
where $c_\mathrm{true}$ is the target model (without noise) 
displayed in \cref{fig:models:true} and $c_\mathrm{rec}$ is 
the reconstruction. We give in \cref{table:relative-error:all}
the model error for all cases.

% ==================================================================================
% ----------------------------------------------------------------------------------
% table with all errors
% ----------------------------------------------------------------------------------
% ==================================================================================
%\begin{table}[ht!] \centering
%\caption{Evaluation of the accuracy of the reconstruction with the relative
%         error $\mathfrak{e}$ of \cref{eq:relative-error} depending on the 
%         acquisition setup and the choice of attenuation models to generate
%         the data and to conduct the inversion.}
%\renewcommand\arraystretch{0.9}
%\noindent \begin{tabular}{
%                |>{\raggedright\arraybackslash}p{.20\linewidth}||
%                 >{\raggedleft\arraybackslash}p{.12\linewidth}|
%                 >{\raggedleft\arraybackslash}p{.14\linewidth}|
%                 >{\raggedleft\arraybackslash}p{.12\linewidth}|
%                 >{\raggedleft\arraybackslash}p{.09\linewidth}|
%                 >{\raggedleft\arraybackslash}p{.08\linewidth}|}
%\hline
%model for the data & \multicolumn{5}{c|}{Attenuation model used for inversion} \\ \hline 
%                   & Cole--Cole & Kelvin--Voigt & Kolsky--Futterman & Maxwell & Zener \\ \hline 
%
%\end{tabular}
%\label{table:relative-error:all}
%\end{table}


\renewcommand\arraystretch{1}
\begin{center}\label{table:relative-error:all}
\begin{longtable}{|>{\raggedright\arraybackslash}p{.20\linewidth}||
                 >{\raggedleft\arraybackslash}p{.11\linewidth}|
                 >{\raggedleft\arraybackslash}p{.14\linewidth}|
                 >{\raggedleft\arraybackslash}p{.20\linewidth}|
                 >{\raggedleft\arraybackslash}p{.08\linewidth}|
                 >{\raggedleft\arraybackslash}p{.06\linewidth}|}
\caption{Evaluation of the accuracy of the reconstruction with the relative
         error $\mathfrak{e}$ of \cref{eq:relative-error} depending on the 
         acquisition setup and the choice of attenuation models to generate
         the data and to conduct the inversion.}
\label{table:relative-error:all} \\
\hline
model for the data & \multicolumn{5}{c|}{Attenuation model used for inversion}        \\ \hline 
                   & Cole--Cole & Kelvin--Voigt & Kolsky--Futterman & Maxwell & Zener \\ \hline \hline
\endfirsthead
  \multicolumn{6}{c}{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\ \hline
\endhead
%% \hline 
  \multicolumn{6}{r}{\textit{Continued on next page}} \\
\endfoot
% \hline % for the very end of the table
\endlastfoot

\multicolumn{6}{c|}{\benchSarRb} \\ \hline 
Cole-Cole          &\arraylineC{1.5064}{0.9821}{0.9536}{1.0349}{0.9779}\\ \hline 
Kelvin--Voigt      &\arraylineC{1.9954}{1.4695}{1.4259}{1.4502}{1.4643}\\ \hline 
Kolsky--Futterman  &\arraylineB{2.0988}{1.5680}{1.6276}{1.6092}{1.5829}\\ \hline 
Maxwell            &\arraylineB{2.0991}{1.5577}{1.7090}{1.7665}{1.5740}\\ \hline 
Zener              &\arraylineC{2.0182}{1.4887}{1.4450}{1.4691}{1.4840}\\ \hline \hline

\multicolumn{6}{c|}{\benchSarRa} \\ \hline 
Cole-Cole          &\arraylineB{1.7110}{1.6810}{1.6870}{1.7469}{1.6786}\\ \hline 
Kelvin--Voigt      &\arraylineE{1.7334}{1.6804}{1.7147}{1.7774}{1.6797}\\ \hline 
Kolsky--Futterman  &\arraylineE{1.7895}{1.7160}{1.7535}{1.8001}{1.7149}\\ \hline 
Maxwell            &\arraylineB{1.8487}{1.7557}{1.8027}{1.8325}{1.7558}\\ \hline 
Zener              &\arraylineB{1.7444}{1.6801}{1.7135}{1.7822}{1.6836}\\ \hline \hline

\multicolumn{6}{c|}{\benchSarRs} \\ \hline 
Cole-Cole          &\arraylineB{1.2206}{0.9899}{1.0414}{1.1635}{0.9939}\\ \hline 
Kelvin--Voigt      &\arraylineB{1.6363}{1.1709}{1.1755}{1.2140}{1.1843}\\ \hline 
Kolsky--Futterman  &\arraylineB{1.6665}{1.2003}{1.2971}{1.2951}{1.2167}\\ \hline 
Maxwell            &\arraylineB{1.6833}{1.2440}{1.3435}{1.4134}{1.2558}\\ \hline 
Zener              &\arraylineB{1.6496}{1.1811}{1.1902}{1.2149}{1.1938}\\ \hline \hline

\multicolumn{6}{c|}{\benchSdkRb} \\ \hline 
Cole-Cole          &\arraylineB{1.3939}{0.8665}{0.8897}{0.9072}{0.8686}\\ \hline 
Kelvin--Voigt      &\arraylineD{1.8624}{1.3860}{1.3940}{1.3843}{1.3851}\\ \hline 
Kolsky--Futterman  &\arraylineB{1.9240}{1.4073}{1.4214}{1.4586}{1.4102}\\ \hline 
Maxwell            &\arraylineB{1.9757}{1.4385}{1.4819}{1.5433}{1.4437}\\ \hline 
Zener              &\arraylineE{1.8686}{1.3885}{1.3954}{1.3893}{1.3883}\\ \hline \hline

\multicolumn{6}{c|}{\benchSdkRd} \\ \hline 
Cole-Cole          &\arraylineB{1.6132}{1.0997}{1.1105}{1.1392}{1.1031}\\ \hline 
Kelvin--Voigt      &\arraylineB{2.0672}{1.5798}{1.6033}{1.6187}{1.5843}\\ \hline 
Kolsky--Futterman  &\arraylineB{2.2064}{1.6856}{1.7315}{1.7496}{1.6921}\\ \hline 
Maxwell            &\arraylineB{2.2981}{1.7503}{1.8090}{1.8358}{1.7577}\\ \hline 
Zener              &\arraylineB{2.0781}{1.5868}{1.6130}{1.6324}{1.5917}\\ \hline \hline

\multicolumn{6}{c|}{\benchSskRb} \\ \hline 
Cole-Cole          &\arraylineB{1.4823}{0.8884}{0.9352}{0.9554}{0.9009}\\ \hline 
Kelvin--Voigt      &\arraylineB{1.9123}{1.4192}{1.4949}{1.5216}{1.4292}\\ \hline 
Kolsky--Futterman  &\arraylineB{2.0224}{1.4872}{1.6605}{1.7252}{1.5069}\\ \hline 
Maxwell            &\arraylineB{2.0698}{1.5127}{1.7075}{1.8324}{1.5326}\\ \hline 
Zener              &\arraylineB{1.9263}{1.4304}{1.5162}{1.5467}{1.4438}\\ \hline \hline

\multicolumn{6}{c|}{\benchSskRs} \\ \hline 
Cole-Cole          &\arraylineB{1.3336}{0.6883}{0.7865}{0.8755}{0.7035}\\ \hline 
Kelvin--Voigt      &\arraylineB{1.9158}{1.2738}{1.3694}{1.4287}{1.2972}\\ \hline 
Kolsky--Futterman  &\arraylineB{2.0494}{1.4171}{1.5627}{1.6448}{1.4408}\\ \hline 
Maxwell            &\arraylineB{2.1179}{1.5165}{1.7001}{1.8132}{1.5398}\\ \hline 
Zener              &\arraylineE{1.9250}{1.2813}{1.3802}{1.4440}{1.3052}\\ \hline \hline

\multicolumn{6}{c|}{\benchSpwRs} \\ \hline 
Cole-Cole          &\arraylineC{1.4425}{1.0385}{0.9928}{0.9978}{1.0375}\\ \hline 
Kelvin--Voigt      &\arraylineD{1.8111}{1.4205}{1.3151}{1.2125}{1.4178}\\ \hline 
Kolsky--Futterman  &\arraylineD{1.8014}{1.3782}{1.3798}{1.2850}{1.3809}\\ \hline 
Maxwell            &\arraylineD{1.7901}{1.3706}{1.3877}{1.3704}{1.3723}\\ \hline 
Zener              &\arraylineD{1.8132}{1.4156}{1.3208}{1.2154}{1.4154}\\ \hline \hline

\multicolumn{6}{c|}{\benchSpwRd} \\ \hline 
Cole-Cole          &\arraylineB{1.2868}{1.0931}{1.1272}{1.1714}{1.0988}\\ \hline 
Kelvin--Voigt      &\arraylineD{1.5336}{1.2341}{1.2251}{1.2536}{1.2368}\\ \hline 
Kolsky--Futterman  &\arraylineD{1.6065}{1.3022}{1.2480}{1.2305}{1.3005}\\ \hline 
Maxwell            &\arraylineD{1.6751}{1.3486}{1.2991}{1.2634}{1.3473}\\ \hline 
Zener              &\arraylineE{1.5387}{1.2343}{1.2247}{1.2491}{1.2349}\\ \hline \hline
\end{longtable}
\end{center}
